Non-cooperative Equilibria of Fermi Systems With Long Range Interactions

We define a Banach space $\mathcal{M}_{1}$ of models for fermions or quantum spins in the lattice with long range interactions and explicit the structure of (generalized) equilibrium states for any $\mathfrak{m}\in \mathcal{M}_{1}$. In particular, we give a first answer to an old open problem in mathematical physics - first addressed by Ginibre in 1968 within a different context - about the validity of the so-called Bogoliubov approximation on the level of states. Depending on the model $\mathfrak{m}\in \mathcal{M}_{1}$, our method provides a systematic way to study all its correlation functions and can thus be used to analyze the physics of long range interactions. Furthermore, we show that the thermodynamics of long range models $\mathfrak{m}\in \mathcal{M}_{1}$ is governed by the non-cooperative equilibria of a zero-sum game, called here the thermodynamic game.

==> firstpage4ams.tex <==
\frontmatter
\title{Non--cooperative Equilibria of Fermi Systems With Long Range
Interactions}

%    Information for first author
\author{J.-B. Bru}
%    Address of record for the research reported here
\address{Departamento de Matem\'{a}ticas, Facultad de Ciencia y
Tecnolog\'{\i}a, Universidad del Pa\'{\i}s Vasco, Apartado 644, 48080 Bilbao,
Spain, and IKERBASQUE, Basque Foundation for Science, 48011, Bilbao, Spain}
%    Current address
\curraddr{Departamento de Matem\'{a}ticas, Facultad de Ciencia y
Tecnolog\'{\i}a, Universidad del Pa\'{\i}s Vasco, Apartado 644, 48080 Bilbao,
Spain}
\email{jb.bru@ikerbasque.org}
%    \thanks will become a 1st page footnote.
\thanks{This work was partially supported by the grant MTM2010-16843 of the
Spanish \textquotedblleft Ministerio de
Ciencia e Innovaci{\'{o}}n\textquotedblright and by
 the \textquotedblleft Inneruniversit{\"{a}}re Forschungsf{\"{o}rderung}%
\textquotedblright\ of the Johannes Gutenberg University in Mainz.}

%    Information for second author
\author{W. de Siqueira Pedra}
\address{Institut f{\"{u}}r Mathematik, Universit{\"{a}}t Mainz,
Staudingerweg 9, 55099 Mainz, Germany}
\email{pedra@mathematik.uni-mainz.de}

\date{October 18, 2010}
\subjclass[2010]{Primary 82B10, 91A40;\\Secondary 46A55, 58E30}
\keywords{Long range interaction, Choquet theorem, equilibrium state, non--cooperative equilibrium, two--person zero--sum game, Bogoliubov approximation, approximating Hamiltonian method, fermion system, quantum spin system}

\begin{abstract}
We define a Banach space $\mathcal{M%
}_{1}$ of models for fermions or quantum spins in the lattice with long range
interactions and explicit the structure of (generalized) equilibrium states
for any $\mathfrak{m}\in \mathcal{M}_{1}$. In particular, we give a first
answer to an old open problem in mathematical physics -- first addressed by
Ginibre in 1968 within a different context -- about
the validity of the so--called Bogoliubov approximation on the level of
states. Depending on the model $\mathfrak{m}\in \mathcal{M}_{1}$, our method
provides a systematic way to study all its correlation functions and can thus be used to analyze the physics of long range interactions.
Furthermore, we show that the thermodynamics of long range
models $\mathfrak{m}\in \mathcal{M}_{1}$ is governed by the non--cooperative equilibria of
a zero--sum game,  called here thermodynamic game.
\end{abstract}

\maketitle

\setcounter{page}{4}
\tableofcontents 
